Multistage Collaborative Knowledge Distillation from a Large Language Model for Semi-Supervised Sequence Generation

We study semi-supervised sequence generation tasks, where the few labeled examples are too scarce to finetune a model, and meanwhile, few-shot prompted large language models (LLMs) exhibit room for improvement. In this paper, we present the discovery that a student model distilled from a few-shot prompted LLM can commonly generalize better than its teacher to unseen examples on such tasks. We find that the student is able to learn a general pattern from the high-quality pseudolabels produced by the teacher during knowledge distillation (KD), and favorably not a general pattern from the low-quality pseudolables. Leveraging this discovery, we propose a new method, Multistage Collaborative Knowledge Distillation from an LLM (MCKD), for these tasks. MCKD first few-shot prompts an LLM to produce pseudolabels for unlabeled data. Then at each stage of an iterative KD process, a new pair of students is trained on disjoint partitions of the pseudolabeled data, and produces new and improved pseudolabels for their unseen partitions. We conduct extensive experiments on four syntactic and semantic parsing datasets and show the effectiveness of MCKD for low-resource semi-supervised sequence generation. On CRAFT biomedical parsing, for example, 3-stage MCKD with 50 labeled examples outperforms an LLM teacher and vanilla KD by 7.5% and 3.7% parsing F1, respectively, and matches the performance of supervised finetuning with 500 labeled examples.

==> draft/intro1112.tex <==
%In this paper, we exploit this property through multi-stage knowledge distillation (\ours) with collaborative peers. At each stage of distillation, the student peers are trained on disjoint splits of the pseudo-labeled data, then each student predicts new pseudolabels for the held-out data they were not trained on, incrementally improving the overall quality of the latest pseudo-labels.


%A commonly used technique to improve the performance of a machine learning model trained on a small set of labeled data is synthetic data generation. First, a model is trained on a small set of labeled data. Then, the model is used to generate pseudo-labels on a set of unlabeled data. Finally, a new model is trained on the pseudo-labels. This process is repeated until the model converges, and the overall training pipeline is refered to as self-training or self-distillation. An important step in this pipeline is ``filtering of the pseudo-labels'' as an effort to extract the highest quality ones. This filtering step is typically done by thresholding the model's confidence on the pseudo-labels, although this can be challenging and often some of the good is thrown away with the bad.

Large language models (LLMs) have shown remarkable performance on many language tasks due to effective in-context learning (ICL). ICL enables rapid domain adaptations using only a few exemplars and is doubly beneficial when annotated data are expensive to obtain. Despite their efficacy, such models are impractical for real world deployment since they are often hosted behind proprietary APIs, expensive, and slow.  {For instance, our approximation is it would cost more than \$10M USD to parse all of Pubmed using prompting.\footnote{There are more than 35M papers on Pubmed. We conservatively estimate it would take at least 20 API calls per paper, and each call would have 1K or more tokens. Currently OpenAI's most powerful model (GPT-4) charges \$0.03 per 1K tokens.} More feasible solutions are thus needed.}  In response, knowledge distillation \cite{hinton2015distilling} has emerged as a promising solution to transfer knowledge from LLMs to smaller, more efficient counterparts. 

%LLM prompting may not require so many labeled data to serve as a strong parser, but is far too expensive to deploy. 

%In this paper, we look into KD from LLMs in low-data regimes, especially for tasks challenging to LLMs.  We use few-shot constituency parsing as the testbed since the task is difficult to learn using a small set of training instances and is a core part of many real world NLP systems. In biomedical texts, for instance, syntactic structures can be used to determine protein-protein interactions~\cite{kanerva2020dependency}. On the other, it took 80 annotators around 2.5 years to parse the 20k sentences of biomedical text in the CRAFT corpus~\cite{verspoor2012corpus}. %


However, LLMs may perform poorly in some tasks potentially because the target distribution is more foreign to their training data. {E.g., LLMs may not perform well in parsing to capture compositional structures due to their incapability in compositional generalization~\citep{drozdov_compositional,keysers2020measuring}.}  In this case, there lacks effective method for few-shot tasks.  Unreliable teacher labels may challenge the viability of the use of KD in this case.

%Since we focus on the few-shot settings where model performance is usually much lower than that with full supervision, we seek techniques to improve the student accuracy as much as possible.
%{ We are motivated to ask, \textit{can we still train a light but decent student model in low-data regimes through KD for tasks that teacher LLMs may not perform reliably?} We first investigate the performance of students with different levels of training fidelity, i.e., the extent that the student is matched to the teacher on a distillation set, and effects of size of distillation set, i.e., size of teacher labels used for training.  We find that the student model that have memorized sufficient teacher labels during KD can outperform the teacher on held-out data, especially in cases where the teacher makes more mistakes.}

%Self-distillation \cite{yarowsky-1995-unsupervised} is the type of knowledge distillation where the teacher and the student are of the same architecture, and can yield improved performance. However, it remains unclear how sequence-level knowledge distillation (SLKD) \citep{kim-rush-2016-sequence} from an LLM can be followed by self-distillation (SD). If the student predictions match the teacher's during SLKD, leveraging the student as the teacher in SD to train another student of the same architecture is effectively a repetition of the SLKD step.

%is a setting of knowledge distillation where the teacher and student are of the same architecture type and model size, and can yield a stronger model than single model training.
% Not all teacher labels are equally informative, and this is especially the case for data the teacher wasn't trained on. Data selection techniques are effective for removing noise from teacher labels and leads to more effective student training.

%Since we focus on the few-shot settings where model performance is usually much lower than that with full supervision, we seek techniques to improve the student accuracy as much as possible.
%{ We are motivated to ask, \textit{can we still train a light but decent student model in low-data regimes through KD for tasks that teacher LLMs may not perform reliably?} We first investigate the performance of students with different levels of training fidelity, i.e., the extent that the student is matched to the teacher on a distillation set, and effects of size of distillation set, i.e., size of teacher labels used for training.  We find that the student model that have memorized sufficient teacher labels during KD can outperform the teacher on held-out data, especially in cases where the teacher makes more mistakes.}

%Self-distillation \cite{yarowsky-1995-unsupervised} is the type of knowledge distillation where the teacher and the student are of the same architecture, and can yield improved performance. However, it remains unclear how sequence-level knowledge distillation (SLKD) \citep{kim-rush-2016-sequence} from an LLM can be followed by self-distillation (SD). If the student predictions match the teacher's during SLKD, leveraging the student as the teacher in SD to train another student of the same architecture is effectively a repetition of the SLKD step.

%is a setting of knowledge distillation where the teacher and student are of the same architecture type and model size, and can yield a stronger model than single model training.
% Not all teacher labels are equally informative, and this is especially the case for data the teacher wasn't trained on. Data selection techniques are effective for removing noise from teacher labels and leads to more effective student training.
% TODO: Add citations.
%Despite the We find that the student model that have memorized sufficient teacher labels during KD can outperform the teacher on held-out data, especially in cases where the teacher makes more mistakes.

 %We show that the Stage 1 students perform better than the teacher on the data they label for the Stage 2 student.

% TODO: Add citations.
Despite the We find that the student model that have memorized sufficient teacher labels during KD can outperform the teacher on held-out data, especially in cases where the teacher makes more mistakes.
We therefore propose a new approach called multi-stage \textbf{P}ee\textbf{R} c\textbf{O}llaborati\textbf{VE} \textbf{K}nowledge \textbf{D}istillation (\ours) that leverages the ability that student can outperform its teacher on held-out data. In the initial stage, an LLM-based teacher model uses few-shot prompting to produce many teacher pseudo labels. In Stage 1 of knowledge distillation, two peer students are trained on separate halves of the teacher's pseudo labels, and each predict labels for the half it was not trained on. In Stage 2, a final student is trained on a union of the student pseudo labels from the previous stage. %We show that the Stage 1 students perform better than the teacher on the data they label for the Stage 2 student.

Our main contributions are as follows.
\begin{itemize}
    \item We investigate knowledge distillation from LLMs in low-data regimes, especially for tasks that LLMs cannot perform reliably.  We propose \ours, a novel variant of knowledge distillation for few-shot settings, which leverages self-distillation to achieve much stronger performance than vanilla KD.
    \item Empirically, our final T5-Base \citep{raffel2020t5} students achieve 15.2\% and 22.3\% error reduction compared to the initial ChatGPT  \citep{chatgpt} teacher on Penn Treebank (English news data) and CRAFT (biomedical text) datasets, while being significantly faster. It takes approximately 24 hours to collect the initial Penn Treebank teacher labels using the ChatGPT API, while T5-base can label the same amount of data in less than 30 mins.
    \item Our analysis suggests that despite the flaws in teacher labels, a student that has memorized sufficient teacher labels during KD can outperform rather than converge to the teacher on held-out data mainly by avoiding repeating the teacher's mistakes.

\end{itemize}


\if 0
{This section first investigates KD from LLMs in low-data regimes, focusing on the student models' generalization performance compared with the teacher model, and then introduces a stronger KD method, i.e., multi-stage KD. }

\subsection{Knowledge Distillation from LLMs in Low-data Regimes}
\label{sec:method_kd}
KD from LLMs is helpful in low-data regimes to train a small deployable model.  But LLMs may perform poorly in some tasks, making themselves unreliable teachers.  {To maximize the effectiveness of KD in this case, we first conduct experiments to investigate an important question \textit{can we still train a light but decent student model in low-data regimes through KD for tasks that teacher LLMs may not perform reliably?} The benefits of KD may be limited if the student cannot even outperform the teacher due to unreliable teacher labels.  We therefore study the performance of students with different levels of training fidelity, i.e., the extent that the student is matched to the teacher on a distillation set (Section~\ref{sec:fidelity}), and effects of size of distillation set, i.e., size of teacher labels used for training (Section~\ref{sec:size}).}
\fi
%tasks
%(1) How to guide the KD process without validation data in low-data regimes? A labeled validation set is usually needed to prevent the model from overfitting training data and having poor generalization performance.  To investigate this in the context of distillation from LLMs, we record the student's training curve wrt. teacher labels and its evaluation curve on held-out data during KD.  
%(2) Can student match or surpass the teacher on heldout dataset? if so, under waht condition
 1. The novelty of the work is not in the concept of multi-stage distillation (which already exists in the literature) but in the specific way it is done: iteratively with pairs of collaborative models — the title, abstract and intro should all reflect this. The title can for example be something like: “Multi-Stage Distillation of Large Language Models with Collaborative Peers”
2. Given the current set of experiments, it might make sense to put the work in a more specific (and somewhat unique) context: not just low-resource, but also where the target distribution is relatively foreign to the LLM (constituency parses). This would make the “student does better than the teacher” narrative more relevant because now there is one more reason for distillation (beyond efficiency and deployability) — training a better model than the teacher, which may be OK, but not perfect, for the task
3. The main RQ should not be if we can match/outperform the teacher (accounts of which can also be found in the existing KD literature), but  more generally can we train good models (that are also lightweight and fast) in few-shot settings by leveraging an original LLM teacher despite the latter not being an ideal model for the task
4. In Sections 2 and 4, the write-up/argument should follow the same order: (1) When distilled with high fidelity, students can generalize better than their teachers (especially on the tasks being considered), and (2) It therefore makes sense to try to distill from them further. 
5. About KD + SD w/ HC: Did you try w/o HC? Because (my understanding is that) HC is not in Mist-KD. I personally feel that this is a confounding factor that is not adding value. I would just do w/o HC for KD + SD.
6. The rationale for the proposed algorithm, especially for labeling the data with students trained on a different partition, should be clearer and more explicit in the Introduction
